SystolicAttention: Fusing FlashAttention within a Single Systolic Array

Transformer models rely heavily on the scaled dot-product attention (SDPA) operation, typically implemented as FlashAttention. Characterized by its frequent interleaving of matrix multiplications and softmax operations, FlashAttention fails to fully utilize the compute resources of modern systolic-array-based accelerators designed for consecutive and large matrix multiplications. To fully unleash the performance potential of systolic arrays for FlashAttention, we propose FSA, an enhanced systolic array architecture that runs the entire FlashAttention on the array without external vector units. Combined with SystolicAttention, an optimized kernel for FSA that achieves fine-grained and element-wise overlapping of FlashAttention operations, FSA maximizes array utilization while preserving the original floating-point operation order of FlashAttention. We implement FSA in synthesizable RTL and evaluate its performance against state-of-the-art systolic-array-based accelerators. Our results show that FSA achieves 1.77x and 4.83x higher attention FLOPs/s utilization compared to AWS Neuron-v2 and Google TPUv5e, respectively. We synthesize FSA in a 16 nm technology at 1.5 GHz, and results indicate only a 12% area overhead compared to a standard weight-stationary systolic array.

==> 8-discussion.tex <==
\section{Discussion}





\subsection{Necessity of a Vector Unit}

While \MSAGA{} is capable of executing \FA{} entirely on the
systolic array without relying on a vector unit, a vector unit or
SFU is still necessary in a full
accelerator system to support activation functions outside of \FA{}.
However, because \MSAGA{} offloads all attention-related computation
from the vector unit, the overall vector \FLOPs{} requirement may be
significantly reduced.





\subsection{Limitations of \MSAGA{}}

Although \MSAGA{} delivers high \FLOPs{} utilization for \FA{},
it is not well-suited for the decoding phase of LLM inference.

\MSAGA{} is ideal for the (1) LLM training and (2) prefill phase of LLM inference,
where the query matrix $Q$ has a long sequence length, making the
attention computation compute-intensive~\cite{splitwise}. In this case, the high
\FLOPs{} throughput of \MSAGA{} effectively accelerates the workload.

In contrast, during the decoding phase, the query $Q$ has a
sequence length of 1, making the computation memory-bound.
Moreover, since \MSAGA{} operates on $128 \times 128$ tiles,
$Q$ must be padded to fit this shape, resulting in substantial
wasted computation and inefficient resource usage.


